The Residual Spectrum of $F_4$ Arising from Degenerate Eisenstein Series

Let $G$ be a split group of type $F_4$ defined over a number field. We study the square-integrable automorphic representations of $G$ that can be realized as leading terms of degenerate Eisenstein series associated to various maximal parabolic subgroups. These representations appear in the residual spectrum. The local representation theory over finite places plays a central role in our work.

==> Tables/p3_holo_table_1.tex <==
  \newpage
 
 \begin{landscape} 
 \renewcommand*{\arraystretch}{1.5} 
 \fontsize{10}{12}
  \begin{longtable}{|L|R|c|c|c|} 
  \hline
 Type & $w$ &  $\dim \Sigma_{w}^{\iwhaori}$  & Exp & Const \\ \hline 
 $H$ & $ w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $ & -- \\ \hline 
 $H$ & $ w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $  & --\\ \hline 
 $H$ & $ w_{3}w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $ & --\\ \hline 
 $H$ & $ w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $ & -- \\ \hline 
 $H$ & $ w_{3}w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $ & -- \\ \hline 
 $H$ & $ w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $ & -- \\ \hline 
 $H$ & $ w_{2}w_{3}w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $ & -- \\ \hline 
 $H$ & $ w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $ & -- \\ \hline 
 $H$ & $ w_{2}w_{3}w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $ & -- \\ \hline 
 $H$ & $ w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $  & --\\ \hline 
 $H$ & $ w_{1}w_{2}w_{3}w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $  & --\\ \hline 
 $H$ & $ w_{1}w_{2}w_{3}w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, 0, -1, 0\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, -1, 1, -1\right] $  & --\\ \hline 
 $H$ & $ w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, -1, 1, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, -1, 1, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, -1, 1, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, -1, 1, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{1}w_{2}w_{3} $ &  42  & $ \left[0, -1, 1, -1\right] $ & -- \\ \hline 
 $HZH$ & $ \left(w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4} \right) \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}\right) $ &  42  & $ \left[0, -1, 1, -1\right] $ & -- \\ \hline 
 $HZH$ & $ \left(w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}\right) 
   \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3} \right)$ &  42  & $ \left[0, -1, 1, -1\right] $ & -- \\ \hline 
 $ZH$ & $ \left(w_{3}w_{2}w_{3}\right) \cdot \left(w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} \right) $ &  42  & $ \left[0, -1, 1, -1\right] $ & -- \\ \hline 
 $ZH$ & $ \left(w_{3}w_{1}w_{2}w_{3}\right)\cdot \left(w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} \right) $ &  42  & $ \left[0, -1, 1, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[-1, 1, -1, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[-1, 1, -1, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{1}w_{2}w_{3} $ &  42  & $ \left[-1, 1, -1, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{2}w_{3} $ &  42  & $ \left[-1, 1, -1, -1\right] $ & --\\ \hline 
 $HZH$ & $ \left(w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}\right) \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3} \right)$ &  42  & $ \left[-1, 1, -1, -1\right] $ & -- \\ \hline
 $HZHZHZH$ & $ w_{2} w_{3}w_{1}w_{2}w_{3} w_{4}w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[-1, 1, -1, -1\right] $  & --\\ \hline 
 $H$ & $ w_{4}w_{3}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[1, 0, -1, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{3}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  42  & $ \left[1, 0, -1, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  61  & $ \left[0, -1, 0, 1\right] $ & $1$ \\ \hline 
 $H$ & $ w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  61  & $ \left[0, -1, 0, 1\right] $ & $1$ \\ \hline 
 $H$ & $ w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  61  & $ \left[0, -1, 0, 1\right] $ & $1$ \\ \hline 
 $H$ & $ w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  61  & $ \left[0, -1, 0, 1\right] $ & $1$ \\ \hline 
 $HZHZH$ & $ \left( w_{2}w_{3}w_{4}\right) \cdot\left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}w_{4}\right) 
   \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[0, -1, 0, 1\right] $ & $-3$ \\ \hline 
 $HZHZH$ & $ \left(w_{1}w_{2}w_{3}w_{4}\right) \cdot\left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}w_{4}\right) 
   \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3} \right) $ &  61  & $ \left[0, -1, 0, 1\right] $ &$-3$ \\ \hline 
 $HZHZH$ & $ \left( w_{3}w_{2}w_{3}w_{4}\right) \cdot\left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}w_{4}\right) 
   \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3} \right) $ &  61  & $ \left[0, -1, 0, 1\right] $ & $-3$ \\ \hline 
 $HZHZH$ & $ \left(w_{3}w_{1}w_{2}w_{3}w_{4}\right) \cdot\left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}w_{4}\right) 
   \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[0, -1, 0, 1\right] $ & $-3$\\ \hline 
 $H$ & $ w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  61  & $ \left[-1, 1, -2, 1\right] $ &$1$ \\ \hline 
 $H$ & $ w_{3}w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  61  & $ \left[-1, 1, -2, 1\right] $ & $1$\\ \hline 
 $H$ & $ w_{3}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{2}w_{3} $ &  61  & $ \left[-1, 1, -2, 1\right] $& $1$ \\ \hline 
 $HZHZH$ & $ 
 \left(
 w_{3}w_{4}\right) \cdot\left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}w_{4}\right) 
   \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[-1, 1, -2, 1\right] $ & $-3$ \\ \hline 
 $ZHZHZH$ & $ \left(w_{2}w_{3}w_{1}w_{2}\right) \cdot\left(w_{3}w_{4}\right) \cdot\left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}w_{4}\right) 
   \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[-1, 1, -2, 1\right] $ &$-3$\\ \hline 
 $H$ & $ w_{4}w_{3}w_{1}w_{2}w_{3}w_{4}w_{1}w_{2}w_{3} $ &  61  & $ \left[-1, 0, 1, -2\right] $  &$1$\\ \hline 
 $H$ & $ w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{1}w_{2}w_{3} $ &  61  & $ \left[-1, 0, 1, -2\right] $ &$1$\\ \hline 
 $HZH$ & $ \left(w_{4}w_{3}w_{1}w_{2}w_{3}w_{4}\right) \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[-1, 0, 1, -2\right] $ &$-1$\\ \hline 
 $HZH$ & $ \left(w_{4}w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}\right) \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[-1, 0, 1, -2\right] $ &$-1$\\ \hline 
 $H$ & $ w_{3}w_{1}w_{2}w_{3}w_{4}w_{1}w_{2}w_{3} $ &  61  & $ \left[-1, 0, -1, 2\right] $ &$1$\\ \hline 
 $H$ & $ w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{1}w_{2}w_{3} $ &  61  & $ \left[-1, 0, -1, 2\right] $  &$1$\\ \hline 
 $HZH$ & $ \left(w_{3}w_{1}w_{2}w_{3}w_{4}\right) \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[-1, 0, -1, 2\right] $ &$-1$\\ \hline 
 $HZH$ & $ \left(w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}\right) \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[-1, 0, -1, 2\right] $ &$-1$\\ \hline 
 $H$ & $ w_{1}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  61  & $ \left[-1, -1, 2, -1\right] $ & $1$\\ \hline 
 $H$ & $ w_{1}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  61  & $ \left[-1, -1, 2, -1\right] $ &$1$ \\ \hline 
 $H$ & $ w_{2}w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{2}w_{3} $ &  61  & $ \left[-1, -1, 2, -1\right] $ &$1$ \\ \hline 
 $HZHZH$ & $ \left(w_{4}\right) \cdot\left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}w_{4}\right) 
   \cdot \left(w_{3}w_{2}w_{3}\right) 
   \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[-1, -1, 2, -1\right] $ &$-3$\\ \hline 
 $HZHZHZH$ & $ \left(w_{3}\right) 
   \cdot \left(w_{2}w_{3}
 w_{1}w_{2}\right) 
   \cdot \left(w_{3}w_{4}\right) \cdot\left(w_{3}w_{2}w_{3}\right) 
  \cdot \left(w_{1}w_{2}w_{3}w_{4}\right) 
  \cdot \left(w_{3}w_{2}w_{3}\right) 
  \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[-1, -1, 2, -1\right] $ &$-3$\\ \hline 
 $H$ & $ w_{4}w_{3}w_{2}w_{3}w_{4}w_{1}w_{2}w_{3} $ &  61  & $ \left[1, -1, 1, -2\right] $ & $1$\\ \hline 
 $HZH$ & $ \left(w_{4}w_{3}w_{2}w_{3}w_{4}\right) \cdot \left(w_{3}w_{2}w_{3}\right) 
  \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[1, -1, 1, -2\right] $ &$-1$\\ \hline 
 $H$ & $ w_{3}w_{2}w_{3}w_{4}w_{1}w_{2}w_{3} $ &  61  & $ \left[1, -1, -1, 2\right] $ &$1$ \\ \hline 
 $HZH$ & $\left( w_{3}w_{2}w_{3}w_{4}\right) \cdot \left(w_{3}w_{2}w_{3}\right) 
  \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[1, -1, -1, 2\right] $ &$-1$\\ \hline 
 $H$ & $ w_{1}w_{2}w_{3}w_{4}w_{1}w_{2}w_{3} $ &  61  & $ \left[-1, -1, 1, 1\right] $ & -- \\ \hline 
 $HZH$ & $ \left(w_{1}w_{2}w_{3}w_{4}\right) \cdot \left(w_{3}w_{2}w_{3}\right) 
  \cdot \left(w_{1}w_{2}w_{3}\right) $ &  61  & $ \left[-1, -1, 1, 1\right] $ & -- \\ \hline 
 $ZHZH$ & $ \left( w_{3}w_{2}w_{3}\right) 
  \cdot \left(w_{1}w_{2}w_{3}w_{4}\right) 
  \cdot \left(w_{3}w_{2}w_{3}\right) 
  \cdot \left(w_{1}w_{2}w_{3}\right)  $ &  61  & $ \left[-1, -1, 1, 1\right] $ & -- \\ \hline 
 $H$ & $ w_{2}w_{3}w_{4}w_{3}w_{2}w_{3} $ &  86  & $ \left[2, -1, 0, -1\right] $ & --\\ \hline 
 $H$ & $ w_{3}w_{2}w_{3}w_{4}w_{3}w_{2}w_{3} $ &  86  & $ \left[2, -1, 0, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{3}w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  86  & $ \left[1, 0, -2, 1\right] $ & -- \\ \hline 
 $H$ & $ w_{3}w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  86  & $ \left[1, 0, -2, 1\right] $ & -- \\ \hline 
 $H$ & $ w_{2}w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  86  & $ \left[1, -2, 2, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{2}w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  86  & $ \left[1, -2, 2, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{3}w_{4}w_{3}w_{1}w_{2}w_{3} $ &  86  & $ \left[-1, 2, -2, -1\right] $ & --  \\ \hline 
 $H$ & $ w_{3}w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  86  & $ \left[-1, 2, -2, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{3}w_{1}w_{2}w_{3} $ &  86  & $ \left[-1, 0, 2, -3\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{2}w_{3}w_{1}w_{2}w_{3} $ &  86  & $ \left[-1, 0, 2, -3\right] $ & -- \\ \hline 
 $H$ & $ w_{3}w_{1}w_{2}w_{3} $ &  86  & $ \left[-1, 0, -1, 3\right] $ & --\\ \hline 
 $H$ & $ w_{2}w_{3}w_{1}w_{2}w_{3} $ &  86  & $ \left[-1, 0, -1, 3\right] $ & -- \\ \hline 
 $H$ & $ w_{1}w_{2}w_{3}w_{4}w_{3}w_{2}w_{3} $ &  86  & $ \left[-2, 1, 0, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{3}w_{1}w_{2}w_{3}w_{4}w_{3}w_{2}w_{3} $ &  86  & $ \left[-2, 1, 0, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{2}w_{3}w_{4}w_{2}w_{3} $ &  86  & $ \left[2, -1, -1, 1\right] $ & -- \\ \hline 
 $H$ & $ w_{3}w_{4}w_{3}w_{2}w_{3} $ &  86  & $ \left[1, 1, -2, -1\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{3}w_{2}w_{3} $ &  86  & $ \left[1, -1, 2, -3\right] $ & -- \\  \hline 
 $H$ & $ w_{3}w_{2}w_{3} $ &  86  & $ \left[1, -1, -1, 3\right] $ & -- \\ \hline 
 $H$ & $ w_{1}w_{2}w_{3}w_{4}w_{2}w_{3} $ &  86  & $ \left[-2, 1, -1, 1\right] $ & -- \\ \hline 
 $H$ & $ w_{2}w_{3}w_{4}w_{1}w_{2}w_{3} $ &  90  & $ \left[1, -2, 1, 1\right] $ & -- \\ \hline 
 $HZH$ & $ \left(w_{2}w_{3}w_{4}\right) \cdot \left(w_{3}w_{2}w_{3}\right) 
  \cdot \left(w_{1}w_{2}w_{3}\right) $ &  90  & $ \left[1, -2, 1, 1\right] $ & -- \\ \hline 
 $H$ & $ w_{3}w_{4}w_{1}w_{2}w_{3} $ &  90  & $ \left[-1, 2, -3, 1\right] $ & -- \\  \hline 
 $HZH$ & $\left( w_{3}w_{4}\right) \cdot \left(w_{3}w_{2}w_{3}\right) 
  \cdot \left(w_{1}w_{2}w_{3}\right) $ &  90  & $ \left[-1, 2, -3, 1\right] $ & -- \\  \hline 
 $H$ & $ w_{4}w_{1}w_{2}w_{3} $ &  90  & $ \left[-1, -1, 3, -2\right] $ & --\\ \hline 
 $HZH$ & $ \left(w_{4}\right) \cdot \left(w_{3}w_{2}w_{3}\right) 
  \cdot \left(w_{1}w_{2}w_{3}\right) $ &  90  & $ \left[-1, -1, 3, -2\right] $ & --\\ \hline 
 $H$ & $ w_{1}w_{2}w_{3} $ &  90  & $ \left[-1, -1, 1, 2\right] $ & -- \\ \hline 
 $ZH$ & $ \left(w_{3}w_{2}w_{3}\right) 
 \cdot \left( w_{1}w_{2}w_{3}\right) $ &  90  & $ \left[-1, -1, 1, 2\right] $ & --\\ \hline 
 $H$ & $ w_{3}w_{4}w_{2}w_{3} $ &  96  & $ \left[1, 1, -3, 1\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{2}w_{3} $ &  96  & $ \left[1, -2, 3, -2\right] $ & -- \\ \hline 
 $H$ & $ w_{2}w_{3} $ &  96  & $ \left[1, -2, 1, 2\right] $ & -- \\ \hline 
 $H$ & $ w_{4}w_{3} $ &  96  & $ \left[-1, 2, -1, -2\right] $ & --\\ \hline 
 $H$ & $ w_{3} $ &  96  & $ \left[-1, 2, -3, 2\right] $ & -- \\ \hline 
 $H$ & $ 1 $ &  96  & $ \left[-1, -1, 3, -1\right] $ & --  \\ \hline   
  \caption{Images of intertwining operators of $P_3$}
  \label{Table:: P3 ::images} 
  \end{longtable}
  \end{landscape}
